Parallel inexact Newton-Krylov and quasi-Newton solvers for nonlinear elasticity

In this work, we address the implementation and performance of inexact Newton-Krylov and quasi-Newton algorithms, more specifically the BFGS method, for the solution of the nonlinear elasticity equations, and compare them to a standard Newton-Krylov method. This is done through a systematic analysis of the performance of the solvers with respect to the problem size, the magnitude of the data and the number of processors in both almost incompressible and incompressible mechanics. We consider three test cases: Cook's membrane (static, almost incompressible), a twist test (static, incompressible) and a cardiac model (complex material, time dependent, almost incompressible). Our results suggest that quasi-Newton methods should be preferred for compressible mechanics, whereas inexact Newton-Krylov methods should be preferred for incompressible problems. We show that these claims are also backed up by the convergence analysis of the methods. In any case, all methods present adequate performance, and provide a significant speed-up over the standard Newton-Krylov method, with a CPU time reduction exceeding 50% in the best cases.

==> plots/cook-perf-lits.tex <==
\begin{figure}
  \begin{subfigure}[b]{0.245\textwidth}
      \begin{plot}{Dofs}{Total linear iterations}
      \addplot+[fill opacity=0.1, color=\newtoncolor] table [x=dofs, y=tot-krylov, col sep=comma] {data/result-perf-cook-Newton-P1.csv};
      \addplot+[fill opacity=0.1, color=\inexactnewtoncolor] table [x=dofs, y=tot-krylov, col sep=comma] {data/result-perf-cook-Newton-inexact-P1.csv};
      \addplot+[fill opacity=0.1, color=\inexactbfgscolor] table [x=dofs, y=tot-krylov, col sep=comma] {data/result-perf-cook-BFGS-inexact-P1.csv};
      \legend {\newton, \inexactnewton, \inexactbfgs}
    \end{plot}
    \caption{\Pone}
  \end{subfigure}
  \begin{subfigure}[b]{0.245\textwidth}
      \begin{plot}{Dofs}{}
      \addplot+[fill opacity=0.1, color=\newtoncolor] table [x=dofs, y=tot-krylov, col sep=comma] {data/result-perf-cook-Newton-P2.csv};
      \addplot+[fill opacity=0.1, color=\inexactnewtoncolor] table [x=dofs, y=tot-krylov, col sep=comma] {data/result-perf-cook-Newton-inexact-P2.csv};
      \addplot+[fill opacity=0.1, color=\inexactbfgscolor] table [x=dofs, y=tot-krylov, col sep=comma] {data/result-perf-cook-BFGS-inexact-P2.csv};
      \legend {\newton, \inexactnewton, \inexactbfgs}
    \end{plot}
    \caption{\Ptwo}
  \end{subfigure}
  \begin{subfigure}[b]{0.245\textwidth}
      \begin{plot}{Dofs}{Average linear iterations}
      \addplot+[fill opacity=0.1, color=\newtoncolor] table [x=dofs, y=avg-krylov, col sep=comma] {data/result-perf-cook-Newton-P1.csv};
      \addplot+[fill opacity=0.1, color=\inexactnewtoncolor] table [x=dofs, y=avg-krylov, col sep=comma] {data/result-perf-cook-Newton-inexact-P1.csv};
      \addplot+[fill opacity=0.1, color=\inexactbfgscolor] table [x=dofs, y=avg-krylov, col sep=comma] {data/result-perf-cook-BFGS-inexact-P1.csv};
      \legend {\newton, \inexactnewton, \inexactbfgs}
    \end{plot}
    \caption{\Pone}
  \end{subfigure}
  \begin{subfigure}[b]{0.245\textwidth}
      \begin{plot}{Dofs}{}
      \addplot+[fill opacity=0.1, color=\newtoncolor] table [x=dofs, y=avg-krylov, col sep=comma] {data/result-perf-cook-Newton-P2.csv};
      \addplot+[fill opacity=0.1, color=\inexactnewtoncolor] table [x=dofs, y=avg-krylov, col sep=comma] {data/result-perf-cook-Newton-inexact-P2.csv};
      \addplot+[fill opacity=0.1, color=\inexactbfgscolor] table [x=dofs, y=avg-krylov, col sep=comma] {data/result-perf-cook-BFGS-inexact-P2.csv};
      \legend {\newton, \inexactnewton, \inexactbfgs}
    \end{plot}
    \caption{\Ptwo}
  \end{subfigure}
  \caption{Cook test. Comparison of the total (left) and average (right) linear iterations.}
  \label{fig:cook perf lin-its}
\end{figure}


==> plots/cook-perf-nl.tex <==
\begin{figure}
  \begin{subfigure}[b]{0.245\textwidth}
    \begin{plot}{Dofs}{Nonlinear iterations}
      \addplot+[fill opacity=0.1, color=\newtoncolor] table [x=dofs, y=nl-its, col sep=comma] {data/result-perf-cook-Newton-P1.csv};
      \addplot+[fill opacity=0.1, color=\inexactnewtoncolor] table [x=dofs, y=nl-its, col sep=comma] {data/result-perf-cook-Newton-inexact-P1.csv};
      \addplot+[fill opacity=0.1, color=\inexactbfgscolor] table [x=dofs, y=nl-its, col sep=comma] {data/result-perf-cook-BFGS-inexact-P1.csv};
      \legend {\newton, \inexactnewton, \inexactbfgs}
    \end{plot}
    \caption{\Pone}
  \end{subfigure}
  \begin{subfigure}[b]{0.245\textwidth}
    \begin{plot}{Dofs}{}
      \addplot+[fill opacity=0.1, color=\newtoncolor] table [x=dofs, y=nl-its, col sep=comma] {data/result-perf-cook-Newton-P2.csv};
      \addplot+[fill opacity=0.1, color=\inexactnewtoncolor] table [x=dofs, y=nl-its, col sep=comma] {data/result-perf-cook-Newton-inexact-P2.csv};
      \addplot+[fill opacity=0.1, color=\inexactbfgscolor] table [x=dofs, y=nl-its, col sep=comma] {data/result-perf-cook-BFGS-inexact-P2.csv};
      \legend {\newton, \inexactnewton, \inexactbfgs}
    \end{plot}
    \caption{\Ptwo}
  \end{subfigure}
  \begin{subfigure}[b]{0.245\textwidth}
    \begin{plot}{Dofs}{}
      \addplot+[fill opacity=0.1, color=\bfgscolor] table [x=dofs, y=nl-its, col sep=comma] {data/result-perf-cook-BFGS-P1.csv};
      \legend {\bfgs}
    \end{plot}
  \caption{\Pone}
  \end{subfigure}
  \begin{subfigure}[b]{0.245\textwidth}
    \begin{plot}{Dofs}{}
      \addplot+[fill opacity=0.1, color=\bfgscolor] table [x=dofs, y=nl-its, col sep=comma] {data/result-perf-cook-BFGS-P2.csv};
      \legend {\bfgs}
    \end{plot}
  \caption{\Ptwo}
  \end{subfigure}

  \caption{Cook test. Comparison of the nonlinear iterations. Two plots are presented, as the BFGS iterations (right) are two orders of magnitude larger than the other methods.}
  \label{fig:cook perf nl-its}
\end{figure}


==> plots/cook-perf-time.tex <==
\begin{figure}
  \centering
  \begin{subfigure}[b]{0.448\textwidth}
      \begin{loglogplot}[height=5cm]{Dofs}{Time (s)}
      \addplot+[fill opacity=0.1, color=\newtoncolor] table [x=dofs, y=time, col sep=comma] {data/result-perf-cook-Newton-P1.csv};
      \addplot+[fill opacity=0.1, color=\inexactnewtoncolor] table [x=dofs, y=time, col sep=comma] {data/result-perf-cook-Newton-inexact-P1.csv};
      \addplot+[fill opacity=0.1, color=\bfgscolor] table [x=dofs, y=time, col sep=comma] {data/result-perf-cook-BFGS-P1.csv};
      \addplot+[fill opacity=0.1, color=\inexactbfgscolor] table [x=dofs, y=time, col sep=comma] {data/result-perf-cook-BFGS-inexact-P1.csv};
      \legend {\newton, \inexactnewton, \bfgs, \inexactbfgs}
    \end{loglogplot}
    \caption{\Pone}
  \end{subfigure}
  \begin{subfigure}[b]{0.448\textwidth}
    \begin{loglogplot}[height=5cm]{Dofs}{}
    \addplot+[fill opacity=0.1, color=\newtoncolor] table [x=dofs, y=time, col sep=comma] {data/result-perf-cook-Newton-P2.csv};
    \addplot+[fill opacity=0.1, color=\inexactnewtoncolor] table [x=dofs, y=time, col sep=comma] {data/result-perf-cook-Newton-inexact-P2.csv};
    \addplot+[fill opacity=0.1, color=\bfgscolor] table [x=dofs, y=time, col sep=comma] {data/result-perf-cook-BFGS-P2.csv};
    \addplot+[fill opacity=0.1, color=\inexactbfgscolor] table [x=dofs, y=time, col sep=comma] {data/result-perf-cook-BFGS-inexact-P2.csv};
    \legend {\newton, \inexactnewton, \bfgs, \inexactbfgs}
  \end{loglogplot}
  \caption{\Ptwo}
  \end{subfigure}
  \caption{Cook test. CPU times plotted with respect to the degrees of freedom.}
  \label{fig:cook perf time}
\end{figure}


==> plots/cook-robust-l.tex <==
\begin{figure}
  \begin{subfigure}[b]{0.45\textwidth}
      \begin{plot}{$\tau$}{Total linear itst}
      \addplot+[fill opacity=0.1, color=\newtoncolor] table [x=rob-param, y=tot-krylov, col sep=comma] {data/result-rob-cook-Newton-P1.csv};
      \addplot+[fill opacity=0.1, color=\inexactnewtoncolor] table [x=rob-param, y=tot-krylov, col sep=comma] {data/result-rob-cook-Newton-inexact-P1.csv};
      \addplot+[fill opacity=0.1, color=\inexactbfgscolor] table [x=rob-param, y=tot-krylov, col sep=comma] {data/result-rob-cook-BFGS-inexact-P1.csv};
      \legend {\newton, \inexactnewton, \inexactbfgs}
    \end{plot}
    \caption{\Pone}
  \end{subfigure}
  \begin{subfigure}[b]{0.45\textwidth}
      \begin{plot}{$\tau$}{Total linear itst}
      \addplot+[fill opacity=0.1, color=\newtoncolor] table [x=rob-param, y=tot-krylov, col sep=comma] {data/result-rob-cook-Newton-P2.csv};
      \addplot+[fill opacity=0.1, color=\inexactnewtoncolor] table [x=rob-param, y=tot-krylov, col sep=comma] {data/result-rob-cook-Newton-inexact-P2.csv};
      \addplot+[fill opacity=0.1, color=\inexactbfgscolor] table [x=rob-param, y=tot-krylov, col sep=comma] {data/result-rob-cook-BFGS-inexact-P2.csv};
      \legend {\newton, \inexactnewton, \inexactbfgs}
    \end{plot}
    \caption{\Ptwo}
  \end{subfigure}

  \begin{subfigure}[b]{0.45\textwidth}
      \begin{plot}{$\tau$}{Average linear itst}
      \addplot+[fill opacity=0.1, color=\newtoncolor] table [x=rob-param, y=avg-krylov, col sep=comma] {data/result-rob-cook-Newton-P1.csv};
      \addplot+[fill opacity=0.1, color=\inexactnewtoncolor] table [x=rob-param, y=avg-krylov, col sep=comma] {data/result-rob-cook-Newton-inexact-P1.csv};
      \addplot+[fill opacity=0.1, color=\inexactbfgscolor] table [x=rob-param, y=avg-krylov, col sep=comma] {data/result-rob-cook-BFGS-inexact-P1.csv};
      \legend {\newton, \inexactnewton, \inexactbfgs}
    \end{plot}
    \caption{\Pone}
  \end{subfigure}
  \begin{subfigure}[b]{0.45\textwidth}
      \begin{plot}{$\tau$}{Average linear itst}
      \addplot+[fill opacity=0.1, color=\newtoncolor] table [x=rob-param, y=avg-krylov, col sep=comma] {data/result-rob-cook-Newton-P2.csv};
      \addplot+[fill opacity=0.1, color=\inexactnewtoncolor] table [x=rob-param, y=avg-krylov, col sep=comma] {data/result-rob-cook-Newton-inexact-P2.csv};
      \addplot+[fill opacity=0.1, color=\inexactbfgscolor] table [x=rob-param, y=avg-krylov, col sep=comma] {data/result-rob-cook-BFGS-inexact-P2.csv};
      \legend {\newton, \inexactnewton, \inexactbfgs}
    \end{plot}
    \caption{\Ptwo}
  \end{subfigure}
  \caption{Cook test. comparison of the total (first column) and average (second column) linear iterations on all tests.}
  \label{fig:cook rob lin-its}
\end{figure}


==> plots/cook-robust-nl.tex <==
\begin{figure}
  \begin{subfigure}[b]{0.49\textwidth}
      \begin{semilogxplot}{$\tau$}{Nonlinear iterations}
      \addplot+[fill opacity=0.1, color=\newtoncolor] table [x=rob-param, y=nl-its, col sep=comma] {data/result-rob-cook-Newton-P1.csv};
      \addplot+[fill opacity=0.1, color=\inexactnewtoncolor] table [x=rob-param, y=nl-its, col sep=comma] {data/result-rob-cook-Newton-inexact-P1.csv};
      \addplot+[fill opacity=0.1, color=\bfgscolor] table [x=rob-param, y=nl-its, col sep=comma] {data/result-rob-cook-BFGS-P1.csv};
      \addplot+[fill opacity=0.1, color=\inexactbfgscolor] table [x=rob-param, y=nl-its, col sep=comma] {data/result-rob-cook-BFGS-inexact-P1.csv};
      \legend {\newton, \inexactnewton, \bfgs, \inexactbfgs}
    \end{semilogxplot}
    \caption{\Pone}
  \end{subfigure}
  \begin{subfigure}[b]{0.49\textwidth}
      \begin{semilogxplot}{$\tau$}{Nonlinear iterations}
      \addplot+[fill opacity=0.1, color=\newtoncolor] table [x=rob-param, y=nl-its, col sep=comma] {data/result-rob-cook-Newton-P2.csv};
      \addplot+[fill opacity=0.1, color=\inexactnewtoncolor] table [x=rob-param, y=nl-its, col sep=comma] {data/result-rob-cook-Newton-inexact-P2.csv};
      \addplot+[fill opacity=0.1, color=\bfgscolor] table [x=rob-param, y=nl-its, col sep=comma] {data/result-rob-cook-BFGS-P2.csv};
      \addplot+[fill opacity=0.1, color=\inexactbfgscolor] table [x=rob-param, y=nl-its, col sep=comma] {data/result-rob-cook-BFGS-inexact-P2.csv};
      \legend {\newton, \inexactnewton, \bfgs, \inexactbfgs}
    \end{semilogxplot}
    \caption{\Ptwo}
  \end{subfigure}
  \caption{Cook test. Nonlinear iterations for first order (left) and second order (right) finite elements.}
  \label{fig:cook rob nl-its}
\end{figure}


==> plots/cook-scalab-l.tex <==
\begin{figure}
  \begin{subfigure}{0.49\textwidth}
    \centering
    \begin{subfigure}{0.49\textwidth}
      \begin{semilogxplot}{Cores}{Total linear its.}
      \addplot+[fill opacity=0.1, color=\newtoncolor] table [x=cores, y=tot-krylov, col sep=comma] {data/result-scalab-cook-Newton-P1.csv};
      \addplot+[fill opacity=0.1, color=\inexactnewtoncolor] table [x=cores, y=tot-krylov, col sep=comma] {data/result-scalab-cook-Newton-inexact-P1.csv};
      \addplot+[fill opacity=0.1, color=\inexactbfgscolor] table [x=cores, y=tot-krylov, col sep=comma] {data/result-scalab-cook-BFGS-inexact-P1.csv};
      \legend{\newton, \inexactnewton, \inexactbfgs}
    \end{semilogxplot}
    \end{subfigure}
  	\begin{subfigure}{0.49\textwidth}
  		\begin{semilogxplot}{Cores}{Average linear its.}
  		\addplot+[fill opacity=0.1, color=\newtoncolor] table [x=cores, y=avg-krylov, col sep=comma] {data/result-scalab-cook-Newton-P1.csv};
  		\addplot+[fill opacity=0.1, color=\inexactnewtoncolor] table [x=cores, y=avg-krylov, col sep=comma] {data/result-scalab-cook-Newton-inexact-P1.csv};
  		\addplot+[fill opacity=0.1, color=\inexactbfgscolor] table [x=cores, y=avg-krylov, col sep=comma] {data/result-scalab-cook-BFGS-inexact-P1.csv};
  		\legend{\newton, \inexactnewton, \inexactbfgs}
  	\end{semilogxplot}
  	\end{subfigure}
  \caption{\Pone}
  \end{subfigure}
  \begin{subfigure}{0.49\textwidth}
  \begin{subfigure}{0.49\textwidth}
      \begin{semilogxplot}{Cores}{Total linear its.}
      \addplot+[fill opacity=0.1,color=\newtoncolor] table [x=cores, y=tot-krylov, col sep=comma] {data/result-scalab-cook-Newton-P2.csv};
      \addplot+[fill opacity=0.1,color=\inexactnewtoncolor] table [x=cores, y=tot-krylov, col sep=comma] {data/result-scalab-cook-Newton-inexact-P2.csv};
      \addplot+[fill opacity=0.1,color=\inexactbfgscolor] table [x=cores, y=tot-krylov, col sep=comma] {data/result-scalab-cook-BFGS-inexact-P2.csv};
      \legend{\newton, \inexactnewton, \inexactbfgs}
    \end{semilogxplot}
    \end{subfigure}
  	\begin{subfigure}{0.49\textwidth}
  		\begin{semilogxplot}{Cores}{Average linear its.}
  		\addplot+[fill opacity=0.1, color=\newtoncolor] table [x=cores, y=avg-krylov, col sep=comma] {data/result-scalab-cook-Newton-P2.csv};
  		\addplot+[fill opacity=0.1, color=\inexactnewtoncolor] table [x=cores, y=avg-krylov, col sep=comma] {data/result-scalab-cook-Newton-inexact-P2.csv};
  		\addplot+[fill opacity=0.1, color=\inexactbfgscolor] table [x=cores, y=avg-krylov, col sep=comma] {data/result-scalab-cook-BFGS-inexact-P2.csv};
  		\legend{\newton, \inexactnewton, \inexactbfgs}
  	\end{semilogxplot}
  	\end{subfigure}
  \caption{\Ptwo}
  \end{subfigure}
  \caption{Cook test. Comparison of the total (first column) and average (second column) linear iterations.}
  \label{fig:cook scalab l}
\end{figure}


==> plots/cook-scalab-nl.tex <==
\begin{figure}
  \centering
  \begin{subfigure}{0.49\textwidth}
    \centering
      \begin{subfigure}{0.49\textwidth}
        \begin{semilogxplot}{Cores}{Nonlinear iterations}
        \addplot+[fill opacity=0.1, color=\newtoncolor] table [x=cores, y=nl-its, col sep=comma] {data/result-scalab-cook-Newton-P1.csv};
        \addplot+[fill opacity=0.1, color=\inexactnewtoncolor] table [x=cores, y=nl-its, col sep=comma] {data/result-scalab-cook-Newton-inexact-P1.csv};
        \addplot+[fill opacity=0.1, color=\inexactbfgscolor] table [x=cores, y=nl-its, col sep=comma] {data/result-scalab-cook-BFGS-inexact-P1.csv};
        \legend{\newton, \inexactnewton, \inexactbfgs}
      \end{semilogxplot}
      \end{subfigure}
      \begin{subfigure}{0.49\textwidth}
        \begin{semilogxplot}{Cores}{}
        \addplot+[fill opacity=0.1, color=\bfgscolor] table [x=cores, y=nl-its, col sep=comma] {data/result-scalab-cook-BFGS-P1.csv};
        \legend{\bfgs}
      \end{semilogxplot}
      \end{subfigure}
  \caption{\Pone}
  \end{subfigure}
  \begin{subfigure}{0.49\textwidth}
    \centering
      \begin{subfigure}{0.49\textwidth}
        \begin{semilogxplot}{Cores}{}
        \addplot+[fill opacity=0.1, color=\newtoncolor] table [x=cores, y=nl-its, col sep=comma] {data/result-scalab-cook-Newton-P2.csv};
        \addplot+[fill opacity=0.1, color=\inexactnewtoncolor] table [x=cores, y=nl-its, col sep=comma] {data/result-scalab-cook-Newton-inexact-P2.csv};
        \addplot+[fill opacity=0.1, color=\inexactbfgscolor] table [x=cores, y=nl-its, col sep=comma] {data/result-scalab-cook-BFGS-inexact-P2.csv};
        \legend{\newton, \inexactnewton, \inexactbfgs}
      \end{semilogxplot}
      \end{subfigure}
      \begin{subfigure}{0.49\textwidth}
        \begin{semilogxplot}{Cores}{}
        \addplot+[fill opacity=0.1, color=\bfgscolor] table [x=cores, y=nl-its, col sep=comma] {data/result-scalab-cook-BFGS-P2.csv};
        \legend{\bfgs}
      \end{semilogxplot}
      \end{subfigure}
  \caption{\Ptwo}
  \end{subfigure}
  \caption{Cook test. Nonlinear iterations for all methods.}
  \label{fig:cook scalab nl}
\end{figure}


==> plots/heart-perf-l-p1.tex <==
\begin{figure}
  \centering
  \begin{subfigure}[b]{0.325\textwidth}
      \begin{plot}{Time (s)}{Total linear iterations}
    %   \addplot+[fill opacity=0.1, mark=none] table [x=t, y=l-its, col sep=comma] {data/HEART_PERF_P1_Newton_prolate_h4_v2_ASCII.csv};
    %   \addplot+[fill opacity=0.1, mark=none] table [x=t, y=l-its, col sep=comma] {data/HEART_PERF_P1_Newton_prolate_4mm.csv};
    %   \addplot+[fill opacity=0.1, green!80!black, mark=none] table [x=t, y=l-its, col sep=comma] {data/HEART_PERF_P1_Newton_prolate_h4_v2_ASCII_ref.csv};
      \addplot+[fill opacity=0.1, mark=none] table [x=t, y=l-its, col sep=comma] {data/HEART_PERF_P1_Newton_prolate_4mm_ref.csv};
    %   \legend {mesh 1, mesh 2, mesh 3, mesh 4}
      \legend {mesh 4}
    \end{plot}
    \caption{Newton}
  \end{subfigure}
  \begin{subfigure}[b]{0.325\textwidth}
      \begin{plot}{Time (s)}{}
    %   \addplot+[fill opacity=0.1, mark=none] table [x=t, y=l-its, col sep=comma] {data/HEART_PERF_P1_Newton-inexact_prolate_h4_v2_ASCII.csv};
    %   \addplot+[fill opacity=0.1, mark=none] table [x=t, y=l-its, col sep=comma] {data/HEART_PERF_P1_Newton-inexact_prolate_4mm.csv};
    %   \addplot+[fill opacity=0.1, green!80!black, mark=none] table [x=t, y=l-its, col sep=comma] {data/HEART_PERF_P1_Newton-inexact_prolate_h4_v2_ASCII_ref.csv};
      \addplot+[fill opacity=0.1, mark=none] table [x=t, y=l-its, col sep=comma] {data/HEART_PERF_P1_Newton-inexact_prolate_4mm_ref.csv};
    %   \legend {mesh 1, mesh 2, mesh 3, mesh 4}
      \legend {mesh 4}
    \end{plot}
    \caption{Inexact Newton}
  \end{subfigure}
  \begin{subfigure}[b]{0.325\textwidth}
    \begin{plot}{Time (s)}{}
    %   \addplot+[fill opacity=0.1, mark=none] table [x=t, y=l-its, col sep=comma] {data/HEART_PERF_P1_BFGS-inexact_prolate_h4_v2_ASCII.csv};
    %   \addplot+[fill opacity=0.1, mark=none] table [x=t, y=l-its, col sep=comma] {data/HEART_PERF_P1_BFGS-inexact_prolate_4mm.csv};
    %   \addplot+[fill opacity=0.1, green!80!black, mark=none] table [x=t, y=l-its, col sep=comma] {data/HEART_PERF_P1_BFGS-inexact_prolate_h4_v2_ASCII_ref.csv};
      \addplot+[fill opacity=0.1, mark=none] table [x=t, y=l-its, col sep=comma] {data/HEART_PERF_P1_BFGS-inexact_prolate_4mm_ref.csv};
    %   \legend {mesh 1, mesh 2, mesh 3, mesh 4}
      \legend {mesh 1, mesh 2, mesh 3, mesh 4}
    \end{plot}
    \caption{Inexact BFGS}
  \end{subfigure}

  % Intermest comparisons
  \begin{subfigure}[b]{0.245\textwidth}
      \begin{plot}{Time (s)}{Total linear iterations}
      \addplot+[fill opacity=0.1, mark=none, color=\newtoncolor] table [x=t, y=l-its, col sep=comma] {data/HEART_PERF_P1_Newton_prolate_h4_v2_ASCII.csv};
      \addplot+[fill opacity=0.1, mark=none, color=\inexactnewtoncolor] table [x=t, y=l-its, col sep=comma] {data/HEART_PERF_P1_Newton-inexact_prolate_h4_v2_ASCII.csv};
      \addplot+[fill opacity=0.1, mark=none, color=\inexactbfgscolor] table [x=t, y=l-its, col sep=comma] {data/HEART_PERF_P1_BFGS-inexact_prolate_h4_v2_ASCII.csv};
      \legend {\newton, \inexactnewton, \inexactbfgs}
    \end{plot}
    \caption{Mesh 1}
  \end{subfigure}
  \begin{subfigure}[b]{0.245\textwidth}
      \begin{plot}{Time (s)}{}
        \addplot+[fill opacity=0.1, mark=none, color=\newtoncolor] table [x=t, y=l-its, col sep=comma] {data/HEART_PERF_P1_Newton_prolate_4mm.csv};
        \addplot+[fill opacity=0.1, mark=none, color=\inexactnewtoncolor] table [x=t, y=l-its, col sep=comma] {data/HEART_PERF_P1_Newton-inexact_prolate_4mm.csv};
        \addplot+[fill opacity=0.1, mark=none, color=\inexactbfgscolor] table [x=t, y=l-its, col sep=comma] {data/HEART_PERF_P1_BFGS-inexact_prolate_4mm.csv};
      \legend {\newton, \inexactnewton, \inexactbfgs}
    \end{plot}
    \caption{Mesh 2}
  \end{subfigure}
  \begin{subfigure}[b]{0.245\textwidth}
    \begin{plot}{Time (s)}{}
      \addplot+[fill opacity=0.1, mark=none, color=\newtoncolor] table [x=t, y=l-its, col sep=comma] {data/HEART_PERF_P1_Newton_prolate_h4_v2_ASCII_ref.csv};
      \addplot+[fill opacity=0.1, mark=none, color=\inexactnewtoncolor] table [x=t, y=l-its, col sep=comma] {data/HEART_PERF_P1_Newton-inexact_prolate_h4_v2_ASCII_ref.csv};
      \addplot+[fill opacity=0.1, mark=none, color=\inexactbfgscolor] table [x=t, y=l-its, col sep=comma] {data/HEART_PERF_P1_BFGS-inexact_prolate_h4_v2_ASCII_ref.csv};
      \legend {\newton, \inexactnewton, \inexactbfgs}
    \end{plot}
    \caption{Mesh 3}
  \end{subfigure}
  \begin{subfigure}[b]{0.245\textwidth}
    \begin{plot}{Time (s)}{}
      \addplot+[fill opacity=0.1, mark=none, color=\newtoncolor] table [x=t, y=l-its, col sep=comma] {data/HEART_PERF_P1_Newton_prolate_4mm_ref.csv};
      \addplot+[fill opacity=0.1, mark=none, color=\inexactnewtoncolor] table [x=t, y=l-its, col sep=comma] {data/HEART_PERF_P1_Newton-inexact_prolate_4mm_ref.csv};
      \addplot+[fill opacity=0.1, mark=none, color=\inexactbfgscolor] table [x=t, y=l-its, col sep=comma] {data/HEART_PERF_P1_BFGS-inexact_prolate_4mm_ref.csv};
      \legend {\newton, \inexactnewton, \inexactbfgs}
    \end{plot}
    \caption{Mesh 4}
  \end{subfigure}
  \caption{Heartbeat test. Total Krylov iterations at eact timestep, using \Pone ~elements. In the first row, we stow of the iterations vary within eact method. In the second row, we compare instead the performance for each mesh.}
  \label{fig:heart perf l-its p1}
\end{figure}


==> plots/heart-perf-l-p2.tex <==
\begin{figure}
  \centering
  \begin{subfigure}[b]{0.325\textwidth}
      \begin{plot}{Time (s)}{Total linear iterations}
    %   \addplot+[fill opacity=0.1, mark=none] table [x=t, y=l-its, col sep=comma] {data/HEART_PERF_P2_Newton_prolate_h4_v2_ASCII.csv};
    %   \addplot+[fill opacity=0.1, mark=none] table [x=t, y=l-its, col sep=comma] {data/HEART_PERF_P2_Newton_prolate_4mm.csv};
    %   \addplot+[fill opacity=0.1, green!80!black, mark=none] table [x=t, y=l-its, col sep=comma] {data/HEART_PERF_P2_Newton_prolate_h4_v2_ASCII_ref.csv};
      \addplot+[fill opacity=0.1, mark=none] table [x=t, y=l-its, col sep=comma] {data/HEART_PERF_P2_Newton_prolate_4mm_ref.csv};
    %   \legend {mesh 1, mesh 2, mesh 3, mesh 4}
      \legend {mesh 4}
    \end{plot}
    \caption{Newton}
  \end{subfigure}
  \begin{subfigure}[b]{0.325\textwidth}
      \begin{plot}{Time (s)}{}
    %   \addplot+[fill opacity=0.1, mark=none] table [x=t, y=l-its, col sep=comma] {data/HEART_PERF_P2_Newton-inexact_prolate_h4_v2_ASCII.csv};
    %   \addplot+[fill opacity=0.1, mark=none] table [x=t, y=l-its, col sep=comma] {data/HEART_PERF_P2_Newton-inexact_prolate_4mm.csv};
    %   \addplot+[fill opacity=0.1, green!80!black, mark=none] table [x=t, y=l-its, col sep=comma] {data/HEART_PERF_P2_Newton-inexact_prolate_h4_v2_ASCII_ref.csv};
      \addplot+[fill opacity=0.1, mark=none] table [x=t, y=l-its, col sep=comma] {data/HEART_PERF_P2_Newton-inexact_prolate_4mm_ref.csv};
      \legend {mesh 4}
    %   \legend {mesh 1, mesh 2, mesh 3, mesh 4}
    \end{plot}
    \caption{Inexact Newton}
  \end{subfigure}
  \begin{subfigure}[b]{0.325\textwidth}
    \begin{plot}{Time (s)}{}
    %   \addplot+[fill opacity=0.1, mark=none] table [x=t, y=l-its, col sep=comma] {data/HEART_PERF_P2_BFGS-inexact_prolate_h4_v2_ASCII.csv};
      \addplot+[fill opacity=0.1, mark=none] table [x=t, y=l-its, col sep=comma] {data/HEART_PERF_P2_BFGS-inexact_prolate_4mm.csv};
      % \addplot+[fill opacity=0.1, green!80!black, mark=none] table [x=t, y=l-its, col sep=comma] {data/HEART_PERF_P2_BFGS-inexact_prolate_h4_v2_ASCII_ref.csv};
      % \addplot+[fill opacity=0.1, mark=none] table [x=t, y=l-its, col sep=comma] {data/HEART_PERF_P2_BFGS-inexact_prolate_4mm_ref.csv};
    %   \legend {mesh 1, mesh 2, mesh 3, mesh 4}
      \legend {mesh 2}
    \end{plot}
    \caption{Inexact BFGS}
  \end{subfigure}

  % Intermest comparisons
  \begin{subfigure}[b]{0.245\textwidth}
      \begin{plot}{Time (s)}{Total linear iterations}
      \addplot+[fill opacity=0.1, mark=none, color=\newtoncolor] table [x=t, y=l-its, col sep=comma] {data/HEART_PERF_P2_Newton_prolate_h4_v2_ASCII.csv};
      \addplot+[fill opacity=0.1, mark=none, color=\inexactnewtoncolor] table [x=t, y=l-its, col sep=comma] {data/HEART_PERF_P2_Newton-inexact_prolate_h4_v2_ASCII.csv};
      \addplot+[fill opacity=0.1, mark=none, color=\inexactbfgscolor] table [x=t, y=l-its, col sep=comma] {data/HEART_PERF_P2_BFGS-inexact_prolate_h4_v2_ASCII.csv};
      \legend {\newton, \inexactnewton, \inexactbfgs}
    \end{plot}
    \caption{Mesh 1}
  \end{subfigure}
  \begin{subfigure}[b]{0.245\textwidth}
      \begin{plot}{Time (s)}{}
        \addplot+[fill opacity=0.1, mark=none, color=\newtoncolor] table [x=t, y=l-its, col sep=comma] {data/HEART_PERF_P2_Newton_prolate_4mm.csv};
        \addplot+[fill opacity=0.1, mark=none, color=\inexactnewtoncolor] table [x=t, y=l-its, col sep=comma] {data/HEART_PERF_P2_Newton-inexact_prolate_4mm.csv};
        \addplot+[fill opacity=0.1, mark=none, color=\inexactbfgscolor] table [x=t, y=l-its, col sep=comma] {data/HEART_PERF_P2_BFGS-inexact_prolate_4mm.csv};
      \legend {\newton, \inexactnewton, \inexactbfgs}
    \end{plot}
    \caption{Mesh 2}
  \end{subfigure}
  \begin{subfigure}[b]{0.245\textwidth}
    \begin{plot}{Time (s)}{}
      \addplot+[fill opacity=0.1,   mark=none, color=\newtoncolor] table [x=t, y=l-its, col sep=comma] {data/HEART_PERF_P2_Newton_prolate_h4_v2_ASCII_ref.csv};
      \addplot+[fill opacity=0.1,   mark=none, color=\inexactnewtoncolor] table [x=t, y=l-its, col sep=comma] {data/HEART_PERF_P2_Newton-inexact_prolate_h4_v2_ASCII_ref.csv};
      % \addplot+[fill opacity=0.1, mark=none, color=\inexactbfgscolor] table [x=t, y=l-its, col sep=comma] {data/HEART_PERF_P2_BFGS-inexact_prolate_h4_v2_ASCII_ref.csv};
      \legend {\newton, \inexactnewton, \inexactbfgs}
    \end{plot}
    \caption{Mesh 3}
  \end{subfigure}
  \begin{subfigure}[b]{0.245\textwidth}
    \begin{plot}{Time (s)}{}
      \addplot+[fill opacity=0.1,   mark=none, color=\newtoncolor] table [x=t, y=l-its, col sep=comma] {data/HEART_PERF_P2_Newton_prolate_4mm_ref.csv};
      \addplot+[fill opacity=0.1,   mark=none, color=\inexactnewtoncolor] table [x=t, y=l-its, col sep=comma] {data/HEART_PERF_P2_Newton-inexact_prolate_4mm_ref.csv};
      % \addplot+[fill opacity=0.1, mark=none, color=\inexactbfgscolor] table [x=t, y=l-its, col sep=comma] {data/HEART_PERF_P2_BFGS-inexact_prolate_4mm_ref.csv};
      \legend {\newton, \inexactnewton, \inexactbfgs}
    \end{plot}
    \caption{Mesh 4}
  \end{subfigure}
  \caption{Heartbeat test. Total Krylov iterations at eact timestep, using \Ptwo ~elements. In the first row, we show of the iterations vary within each method. In the second row, we compare instead the performance for each mesh.}
  \label{fig:heart perf l-its p2}
\end{figure}


==> plots/heart-perf-nl-p1.tex <==
\begin{figure}
  \begin{subfigure}[b]{0.245\textwidth}
      \begin{plot}{Time (s)}{Nonlinear iterations}
    %   \addplot+[fill opacity=0.1, mark=none] table [x=t, y=nl-its, col sep=comma] {data/HEART_PERF_P1_Newton_prolate_h4_v2_ASCII.csv};
    %   \addplot+[fill opacity=0.1, mark=none] table [x=t, y=nl-its, col sep=comma] {data/HEART_PERF_P1_Newton_prolate_4mm.csv};
    %   \addplot+[fill opacity=0.1, green!80!black, mark=none] table [x=t, y=nl-its, col sep=comma] {data/HEART_PERF_P1_Newton_prolate_h4_v2_ASCII_ref.csv};
      \addplot+[fill opacity=0.1, mark=none] table [x=t, y=nl-its, col sep=comma] {data/HEART_PERF_P1_Newton_prolate_4mm_ref.csv};
    %   \legend {mesh 1, mesh 2, mesh 3, mesh 4}
      \legend {mesh 4}
    \end{plot}
    \caption{Newton}
  \end{subfigure}
  \begin{subfigure}[b]{0.245\textwidth}
      \begin{plot}{Time (s)}{}
    %   \addplot+[fill opacity=0.1, mark=none] table [x=t, y=nl-its, col sep=comma] {data/HEART_PERF_P1_Newton-inexact_prolate_h4_v2_ASCII.csv};
    %   \addplot+[fill opacity=0.1, mark=none] table [x=t, y=nl-its, col sep=comma] {data/HEART_PERF_P1_Newton-inexact_prolate_4mm.csv};
    %   \addplot+[fill opacity=0.1, green!80!black, mark=none] table [x=t, y=nl-its, col sep=comma] {data/HEART_PERF_P1_Newton-inexact_prolate_h4_v2_ASCII_ref.csv};
      \addplot+[fill opacity=0.1, mark=none] table [x=t, y=nl-its, col sep=comma] {data/HEART_PERF_P1_Newton-inexact_prolate_4mm_ref.csv};
      \legend {mesh 4}
    %   \legend {mesh 1, mesh 2, mesh 3, mesh 4}
    \end{plot}
    \caption{Inexact Newton}
  \end{subfigure}
  \begin{subfigure}[b]{0.245\textwidth}
      \begin{plot}{Time (s)}{}
    %   \addplot+[fill opacity=0.1, mark=none] table [x=t, y=nl-its, col sep=comma] {data/HEART_PERF_P1_BFGS_prolate_h4_v2_ASCII.csv};
    %   \addplot+[fill opacity=0.1, mark=none] table [x=t, y=nl-its, col sep=comma] {data/HEART_PERF_P1_BFGS_prolate_4mm.csv};
    %   \addplot+[fill opacity=0.1, green!80!black, mark=none] table [x=t, y=nl-its, col sep=comma] {data/HEART_PERF_P1_BFGS_prolate_h4_v2_ASCII_ref.csv};
      \addplot+[fill opacity=0.1, mark=none] table [x=t, y=nl-its, col sep=comma] {data/HEART_PERF_P1_BFGS_prolate_4mm_ref.csv};
    %   \legend {mesh 1, mesh 2, mesh 3, mesh 4}
      \legend {mesh 4}
    \end{plot}
    \caption{BFGS}
  \end{subfigure}
  \begin{subfigure}[b]{0.245\textwidth}
    \begin{plot}{Time (s)}{}
    %   \addplot+[fill opacity=0.1, mark=none] table [x=t, y=nl-its, col sep=comma] {data/HEART_PERF_P1_BFGS-inexact_prolate_h4_v2_ASCII.csv};
    %   \addplot+[fill opacity=0.1, mark=none] table [x=t, y=nl-its, col sep=comma] {data/HEART_PERF_P1_BFGS-inexact_prolate_4mm.csv};
    %   \addplot+[fill opacity=0.1, green!80!black, mark=none] table [x=t, y=nl-its, col sep=comma] {data/HEART_PERF_P1_BFGS-inexact_prolate_h4_v2_ASCII_ref.csv};
      \addplot+[fill opacity=0.1, mark=none] table [x=t, y=nl-its, col sep=comma] {data/HEART_PERF_P1_BFGS-inexact_prolate_4mm_ref.csv};
    %   \legend {mesh 1, mesh 2, mesh 3, mesh 4}
      \legend {mesh 4}
    \end{plot}
    \caption{Inexact BFGS}
  \end{subfigure}
  \caption{Heartbeat test. Total nonlinear iterations at each timestep, using \Pone ~elements.}
  \label{fig:heart perf nl p1}
\end{figure}


==> plots/heart-perf-nl-p2.tex <==
\begin{figure}
  \begin{subfigure}[b]{0.245\textwidth}
      \begin{plot}{Time (s)}{Nonlinear iterations}
    %   \addplot+[fill opacity=0.1, mark=none] table [x=t, y=nl-its, col sep=comma] {data/HEART_PERF_P2_Newton_prolate_h4_v2_ASCII.csv};
    %   \addplot+[fill opacity=0.1, mark=none] table [x=t, y=nl-its, col sep=comma] {data/HEART_PERF_P2_Newton_prolate_4mm.csv};
    %   \addplot+[fill opacity=0.1, green!80!black, mark=none] table [x=t, y=nl-its, col sep=comma] {data/HEART_PERF_P2_Newton_prolate_h4_v2_ASCII_ref.csv};
      \addplot+[fill opacity=0.1, mark=none] table [x=t, y=nl-its, col sep=comma] {data/HEART_PERF_P2_Newton_prolate_4mm_ref.csv};
    %   \legend {mesh 1, mesh 2, mesh 3, mesh 4}
      \legend {mesh 4}
    \end{plot}
    \caption{Newton}
  \end{subfigure}
  \begin{subfigure}[b]{0.245\textwidth}
      \begin{plot}{Time (s)}{}
    %   \addplot+[fill opacity=0.1, mark=none] table [x=t, y=nl-its, col sep=comma] {data/HEART_PERF_P2_Newton-inexact_prolate_h4_v2_ASCII.csv};
    %   \addplot+[fill opacity=0.1, mark=none] table [x=t, y=nl-its, col sep=comma] {data/HEART_PERF_P2_Newton-inexact_prolate_4mm.csv};
    %   \addplot+[fill opacity=0.1, green!80!black, mark=none] table [x=t, y=nl-its, col sep=comma] {data/HEART_PERF_P2_Newton-inexact_prolate_h4_v2_ASCII_ref.csv};
      \addplot+[fill opacity=0.1, mark=none] table [x=t, y=nl-its, col sep=comma] {data/HEART_PERF_P2_Newton-inexact_prolate_4mm_ref.csv};
    %   \legend {mesh 1, mesh 2, mesh 3, mesh 4}
      \legend {mesh 4}
    \end{plot}
    \caption{Inexact Newton}
  \end{subfigure}
  \begin{subfigure}[b]{0.245\textwidth}
      \begin{plot}{Time (s)}{}
    %   \addplot+[fill opacity=0.1, mark=none] table [x=t, y=nl-its, col sep=comma] {data/HEART_PERF_P2_BFGS_prolate_h4_v2_ASCII.csv};
    %   \addplot+[fill opacity=0.1, mark=none] table [x=t, y=nl-its, col sep=comma] {data/HEART_PERF_P2_BFGS_prolate_4mm.csv};
    %   \addplot+[fill opacity=0.1, green!80!black, mark=none] table [x=t, y=nl-its, col sep=comma] {data/HEART_PERF_P2_BFGS_prolate_h4_v2_ASCII_ref.csv};
      \addplot+[fill opacity=0.1, mark=none] table [x=t, y=nl-its, col sep=comma] {data/HEART_PERF_P2_BFGS_prolate_4mm_ref.csv};
    %   \legend {mesh 1, mesh 2, mesh 3, mesh 4}
      \legend {mesh 4}
    \end{plot}
    \caption{BFGS}
  \end{subfigure}
  \begin{subfigure}[b]{0.245\textwidth}
    \begin{plot}{Time (s)}{}
    %   \addplot+[fill opacity=0.1, mark=none] table [x=t, y=nl-its, col sep=comma] {data/HEART_PERF_P2_BFGS-inexact_prolate_h4_v2_ASCII.csv};
      \addplot+[fill opacity=0.1, mark=none] table [x=t, y=nl-its, col sep=comma] {data/HEART_PERF_P2_BFGS-inexact_prolate_4mm.csv};
      % \addplot+[fill opacity=0.1, green!80!black, mark=none] table [x=t, y=nl-its, col sep=comma] {data/HEART_PERF_P2_BFGS-inexact_prolate_h4_v2_ASCII_ref.csv};
      % \addplot+[fill opacity=0.1, mark=none] table [x=t, y=nl-its, col sep=comma] {data/HEART_PERF_P2_BFGS-inexact_prolate_4mm_ref.csv};
    %   \legend {mesh 1, mesh 2, mesh 3, mesh 4}
      \legend {mesh 2}
    \end{plot}
    \caption{Inexact BFGS}
  \end{subfigure}
  \caption{Heartbeat test. Total nonlinear iterations at eact timestep, using \Ptwo ~elements. Meshes 3 and 4 tave been discarded from inexact BFGS as they diverged after some time steps. }
  \label{fig:heart perf nl p2}
\end{figure}


==> plots/heart-perf-time-p1.tex <==
\begin{figure}
  \begin{subfigure}[b]{0.245\textwidth}
      \begin{semilogyplot}{Time (s)}{CPU time}
      \addplot+[fill opacity=0.1, mark=none, color=\newtoncolor] table [x=t, y=solution-time, col sep=comma] {data/HEART_PERF_P1_Newton_prolate_h4_v2_ASCII.csv};
      \addplot+[fill opacity=0.1, mark=none, color=\inexactnewtoncolor] table [x=t, y=solution-time, col sep=comma] {data/HEART_PERF_P1_Newton-inexact_prolate_h4_v2_ASCII.csv};
      \addplot+[fill opacity=0.1, mark=none, color=\inexactbfgscolor] table [x=t, y=solution-time, col sep=comma] {data/HEART_PERF_P1_BFGS-inexact_prolate_h4_v2_ASCII.csv};
      \addplot+[fill opacity=0.1, mark=none, color=\bfgscolor] table [x=t, y=solution-time, col sep=comma] {data/HEART_PERF_P1_BFGS_prolate_h4_v2_ASCII.csv};
      \legend {\newton, \inexactnewton, \inexactbfgs, \bfgs}
    \end{semilogyplot}
    \caption{Mesh 1}
  \end{subfigure}
  \begin{subfigure}[b]{0.245\textwidth}
      \begin{semilogyplot}{Time (s)}{}
        \addplot+[fill opacity=0.1, mark=none, color=\newtoncolor] table [x=t, y=solution-time, col sep=comma] {data/HEART_PERF_P1_Newton_prolate_4mm.csv};
        \addplot+[fill opacity=0.1, mark=none, color=\inexactnewtoncolor] table [x=t, y=solution-time, col sep=comma] {data/HEART_PERF_P1_Newton-inexact_prolate_4mm.csv};
        \addplot+[fill opacity=0.1, mark=none, color=\inexactbfgscolor] table [x=t, y=solution-time, col sep=comma] {data/HEART_PERF_P1_BFGS-inexact_prolate_4mm.csv};
        \addplot+[fill opacity=0.1, mark=none, color=\bfgscolor] table [x=t, y=solution-time, col sep=comma] {data/HEART_PERF_P1_BFGS_prolate_4mm.csv};
      \legend {\newton, \inexactnewton, \inexactbfgs, \bfgs}
    \end{semilogyplot}
    \caption{Mesh 2}
  \end{subfigure}
  \begin{subfigure}[b]{0.245\textwidth}
      \begin{semilogyplot}{Time (s)}{}
        \addplot+[fill opacity=0.1, mark=none, color=\newtoncolor] table [x=t, y=solution-time, col sep=comma] {data/HEART_PERF_P1_Newton_prolate_h4_v2_ASCII_ref.csv};
        \addplot+[fill opacity=0.1, mark=none, color=\inexactnewtoncolor] table [x=t, y=solution-time, col sep=comma] {data/HEART_PERF_P1_Newton-inexact_prolate_h4_v2_ASCII_ref.csv};
        \addplot+[fill opacity=0.1, mark=none, color=\inexactbfgscolor] table [x=t, y=solution-time, col sep=comma] {data/HEART_PERF_P1_BFGS-inexact_prolate_h4_v2_ASCII_ref.csv};
        \addplot+[fill opacity=0.1, mark=none, color=\bfgscolor] table [x=t, y=solution-time, col sep=comma] {data/HEART_PERF_P1_BFGS_prolate_h4_v2_ASCII_ref.csv};
      \legend {\newton, \inexactnewton, \inexactbfgs, \bfgs}
    \end{semilogyplot}
    \caption{Mesh 3}
  \end{subfigure}
  \begin{subfigure}[b]{0.245\textwidth}
    \begin{semilogyplot}{Time (s)}{}
      \addplot+[fill opacity=0.1, mark=none, color=\newtoncolor] table [x=t, y=solution-time, col sep=comma] {data/HEART_PERF_P1_Newton_prolate_4mm_ref.csv};
      \addplot+[fill opacity=0.1, mark=none, color=\inexactnewtoncolor] table [x=t, y=solution-time, col sep=comma] {data/HEART_PERF_P1_Newton-inexact_prolate_4mm_ref.csv};
      \addplot+[fill opacity=0.1, mark=none, color=\inexactbfgscolor] table [x=t, y=solution-time, col sep=comma] {data/HEART_PERF_P1_BFGS-inexact_prolate_4mm_ref.csv};
      \addplot+[fill opacity=0.1, mark=none, color=\bfgscolor] table [x=t, y=solution-time, col sep=comma] {data/HEART_PERF_P1_BFGS_prolate_4mm_ref.csv};
      \legend {\newton, \inexactnewton, \inexactbfgs, \bfgs}
    \end{semilogyplot}
    \caption{Mesh 4}
  \end{subfigure}
  \caption{Heartbeat test. CPU time at each timestep, using \Pone ~elements.}
  \label{fig:heart perf time p1}
\end{figure}


==> plots/heart-perf-time-p2.tex <==
\begin{figure}
  \begin{subfigure}[b]{0.245\textwidth}
      \begin{semilogyplot}{Time (s)}{CPU time}
      \addplot+[fill opacity=0.1, mark=none, color=\newtoncolor] table [x=t, y=solution-time, col sep=comma] {data/HEART_PERF_P2_Newton_prolate_h4_v2_ASCII.csv};
      \addplot+[fill opacity=0.1, mark=none, color=\inexactnewtoncolor] table [x=t, y=solution-time, col sep=comma] {data/HEART_PERF_P2_Newton-inexact_prolate_h4_v2_ASCII.csv};
      \addplot+[fill opacity=0.1, mark=none, color=\bfgscolor] table [x=t, y=solution-time, col sep=comma] {data/HEART_PERF_P2_BFGS_prolate_h4_v2_ASCII.csv};
      \addplot+[fill opacity=0.1, mark=none, color=\inexactbfgscolor] table [x=t, y=solution-time, col sep=comma] {data/HEART_PERF_P2_BFGS-inexact_prolate_h4_v2_ASCII.csv};
      \legend {\newton, \inexactnewton, \bfgs, \inexactbfgs}
    \end{semilogyplot}
    \caption{Mesh 1}
  \end{subfigure}
  \begin{subfigure}[b]{0.245\textwidth}
      \begin{semilogyplot}{Time (s)}{}
        \addplot+[fill opacity=0.1, mark=none, color=\newtoncolor] table [x=t, y=solution-time, col sep=comma] {data/HEART_PERF_P2_Newton_prolate_4mm.csv};
        \addplot+[fill opacity=0.1, mark=none, color=\inexactnewtoncolor] table [x=t, y=solution-time, col sep=comma] {data/HEART_PERF_P2_Newton-inexact_prolate_4mm.csv};
        \addplot+[fill opacity=0.1, mark=none, color=\bfgscolor] table [x=t, y=solution-time, col sep=comma] {data/HEART_PERF_P2_BFGS_prolate_4mm.csv};
        \addplot+[fill opacity=0.1, mark=none, color=\inexactbfgscolor] table [x=t, y=solution-time, col sep=comma] {data/HEART_PERF_P2_BFGS-inexact_prolate_4mm.csv};
      \legend {\newton, \inexactnewton, \bfgs, \inexactbfgs}
    \end{semilogyplot}
    \caption{Mesh 2}
  \end{subfigure}
  \begin{subfigure}[b]{0.245\textwidth}
      \begin{semilogyplot}{Time (s)}{}
        \addplot+[fill opacity=0.1,   mark=none, color=\newtoncolor] table [x=t, y=solution-time, col sep=comma] {data/HEART_PERF_P2_Newton_prolate_h4_v2_ASCII_ref.csv};
        \addplot+[fill opacity=0.1,   mark=none, color=\inexactnewtoncolor] table [x=t, y=solution-time, col sep=comma] {data/HEART_PERF_P2_Newton-inexact_prolate_h4_v2_ASCII_ref.csv};
        \addplot+[fill opacity=0.1,   mark=none, color=\bfgscolor] table [x=t, y=solution-time, col sep=comma] {data/HEART_PERF_P2_BFGS_prolate_h4_v2_ASCII_ref.csv};
        % \addplot+[fill opacity=0.1, mark=none, color=\inexactbfgscolor] table [x=t, y=solution-time, col sep=comma] {data/HEART_PERF_P2_BFGS-inexact_prolate_h4_v2_ASCII_ref.csv};
      \legend {\newton, \inexactnewton, \bfgs, \inexactbfgs}
    \end{semilogyplot}
    \caption{Mesh 3}
  \end{subfigure}
  \begin{subfigure}[b]{0.245\textwidth}
    \begin{semilogyplot}{Time (s)}{}
      \addplot+[fill opacity=0.1,   mark=none, color=\newtoncolor] table [x=t, y=solution-time, col sep=comma] {data/HEART_PERF_P2_Newton_prolate_4mm_ref.csv};
      \addplot+[fill opacity=0.1,   mark=none, color=\inexactnewtoncolor] table [x=t, y=solution-time, col sep=comma] {data/HEART_PERF_P2_Newton-inexact_prolate_4mm_ref.csv};
      \addplot+[fill opacity=0.1,   mark=none, color=\bfgscolor] table [x=t, y=solution-time, col sep=comma] {data/HEART_PERF_P2_BFGS_prolate_4mm_ref.csv};
      % \addplot+[fill opacity=0.1, mark=none, color=\inexactbfgscolor] table [x=t, y=solution-time, col sep=comma] {data/HEART_PERF_P2_BFGS-inexact_prolate_4mm_ref.csv};
      \legend {\newton, \inexactnewton, \bfgs, \inexactbfgs}
    \end{semilogyplot}
    \caption{Mesh 4}
  \end{subfigure}
  \caption{Heartbeat test. CPU time at each timestep, using \Ptwo ~elements.}
  \label{fig:heart perf time p2}
\end{figure}


==> plots/heart-robust-dt.tex <==
\begin{figure}
  \begin{subfigure}{0.49\textwidth}
    \begin{tikzpicture}
    \begin{axis}[width=\textwidth, height=5cm, xlabel=Time (s), ylabel=Maximum admissible $\Delta t$, tick label style={font=\footnotesize}, legend style={font=\tiny, draw=none, fill opacity=0.5, text opacity = 1,row sep=2pt},legend columns=2, no markers]
  % \begin{plot}{Time}{Maximum admissible $\Delta t$}
    % Newton P1
    \addplot+[color=\newtoncolor] coordinates {
            (0.01, 0.08) (0.02, 0.09999999999999999) (0.03, 0.12999999999999998) (0.04, 0.36000000000000015) (0.05, 0.35000000000000014) (0.06, 0.3300000000000001) (0.07, 0.3100000000000001) (0.08, 0.3000000000000001) (0.09, 0.2800000000000001) (0.1, 0.2700000000000001) (0.11, 0.25000000000000006) (0.12, 0.24000000000000007) (0.13, 0.22000000000000006) (0.14, 0.21000000000000005) (0.15, 0.20000000000000004) (0.16, 0.19000000000000003) (0.17, 0.17) (0.18, 0.16) (0.19, 0.15) (0.2, 0.13999999999999999) (0.21, 0.12999999999999998) (0.22, 0.11999999999999998) (0.23, 0.10999999999999999) (0.24, 0.09999999999999999) (0.25, 0.09) (0.26, 0.09) (0.27, 0.08) (0.28, 0.07) (0.29, 0.07) (0.3, 0.060000000000000005) (0.31, 0.05) (0.32, 0.05) (0.33, 0.04) (0.34, 0.05) (0.35000000000000003, 0.04) (0.36, 0.03) (0.37, 0.04) (0.38, 0.02) (0.39, 0.4100000000000002) (0.4, 0.4000000000000002) (0.41000000000000003, 0.3900000000000002) (0.42, 0.38000000000000017) (0.43, 0.37000000000000016) (0.44, 0.36000000000000015) (0.45, 0.35000000000000014) (0.46, 0.34000000000000014) (0.47000000000000003, 0.3300000000000001) (0.48, 0.3300000000000001) (0.49, 0.3200000000000001) (0.5, 0.3100000000000001) (0.51, 0.3000000000000001) (0.52, 0.2900000000000001) (0.53, 0.2800000000000001) (0.54, 0.2700000000000001) (0.55, 0.26000000000000006) (0.56, 0.24000000000000007) (0.5700000000000001, 0.23000000000000007) (0.58, 0.23000000000000007) (0.59, 0.22000000000000006) (0.6, 0.21000000000000005) (0.61, 0.20000000000000004) (0.62, 0.19000000000000003) (0.63, 0.18000000000000002) (0.64, 0.17) (0.65, 0.16) (0.66, 0.15) (0.67, 0.13999999999999999) (0.68, 0.12999999999999998) (0.6900000000000001, 0.11999999999999998) (0.7000000000000001, 0.10999999999999999) (0.71, 0.09999999999999999) (0.72, 0.09) (0.73, 0.08) (0.74, 0.07) (0.75, 0.060000000000000005) (0.76, 0.05) (0.77, 0.04) (0.78, 0.03) (0.79, 0.02) (0.8, 0.01)};
  % Newton-inexact P1
  \addplot+[color=\inexactnewtoncolor] coordinates{
  (0.01, 0.09999999999999999) (0.02, 0.10999999999999999) (0.03, 0.7700000000000005) (0.04, 0.7600000000000005) (0.05, 0.7500000000000004) (0.06, 0.7400000000000004) (0.07, 0.7300000000000004) (0.08, 0.3200000000000001) (0.09, 0.3100000000000001) (0.1, 0.3000000000000001) (0.11, 0.2800000000000001) (0.12, 0.2700000000000001) (0.13, 0.25000000000000006) (0.14, 0.24000000000000007) (0.15, 0.23000000000000007) (0.16, 0.22000000000000006) (0.17, 0.21000000000000005) (0.18, 0.19000000000000003) (0.19, 0.18000000000000002) (0.2, 0.17) (0.21, 0.16) (0.22, 0.15) (0.23, 0.13999999999999999) (0.24, 0.12999999999999998) (0.25, 0.12999999999999998) (0.26, 0.11999999999999998) (0.27, 0.10999999999999999) (0.28, 0.09999999999999999) (0.29, 0.09) (0.3, 0.09) (0.31, 0.08) (0.32, 0.08) (0.33, 0.07) (0.34, 0.09999999999999999) (0.35000000000000003, 0.45000000000000023) (0.36, 0.4400000000000002) (0.37, 0.4300000000000002) (0.38, 0.4200000000000002) (0.39, 0.4100000000000002) (0.4, 0.4000000000000002) (0.41000000000000003, 0.3900000000000002) (0.42, 0.38000000000000017) (0.43, 0.37000000000000016) (0.44, 0.36000000000000015) (0.45, 0.35000000000000014) (0.46, 0.34000000000000014) (0.47000000000000003, 0.3300000000000001) (0.48, 0.3300000000000001) (0.49, 0.3200000000000001) (0.5, 0.3100000000000001) (0.51, 0.3000000000000001) (0.52, 0.2900000000000001) (0.53, 0.2800000000000001) (0.54, 0.2700000000000001) (0.55, 0.26000000000000006) (0.56, 0.24000000000000007) (0.5700000000000001, 0.23000000000000007) (0.58, 0.23000000000000007) (0.59, 0.22000000000000006) (0.6, 0.21000000000000005) (0.61, 0.20000000000000004) (0.62, 0.19000000000000003) (0.63, 0.18000000000000002) (0.64, 0.17) (0.65, 0.16) (0.66, 0.15) (0.67, 0.13999999999999999) (0.68, 0.12999999999999998) (0.6900000000000001, 0.11999999999999998) (0.7000000000000001, 0.10999999999999999) (0.71, 0.09999999999999999) (0.72, 0.09) (0.73, 0.08) (0.74, 0.07) (0.75, 0.060000000000000005) (0.76, 0.05) (0.77, 0.04) (0.78, 0.03) (0.79, 0.02) (0.8, 0.01)
  };
  % BFGS P1
  \addplot+[color=\bfgscolor] coordinates {
  (0.01, 0.07) (0.02, 0.060000000000000005) (0.03, 0.07) (0.04, 0.10999999999999999) (0.05, 0.7500000000000004) (0.06, 0.7400000000000004) (0.07, 0.7300000000000004) (0.08, 0.7200000000000004) (0.09, 0.7100000000000004) (0.1, 0.7000000000000004) (0.11, 0.6900000000000004) (0.12, 0.6800000000000004) (0.13, 0.6700000000000004) (0.14, 0.6600000000000004) (0.15, 0.6500000000000004) (0.16, 0.6400000000000003) (0.17, 0.6300000000000003) (0.18, 0.6200000000000003) (0.19, 0.6100000000000003) (0.2, 0.6000000000000003) (0.21, 0.5900000000000003) (0.22, 0.5800000000000003) (0.23, 0.5700000000000003) (0.24, 0.5600000000000003) (0.25, 0.5500000000000003) (0.26, 0.5400000000000003) (0.27, 0.5300000000000002) (0.28, 0.5200000000000002) (0.29, 0.5100000000000002) (0.3, 0.5000000000000002) (0.31, 0.49000000000000027) (0.32, 0.48000000000000026) (0.33, 0.47000000000000025) (0.34, 0.46000000000000024) (0.35000000000000003, 0.45000000000000023) (0.36, 0.4400000000000002) (0.37, 0.4300000000000002) (0.38, 0.4200000000000002) (0.39, 0.4100000000000002) (0.4, 0.4000000000000002) (0.41000000000000003, 0.3900000000000002) (0.42, 0.38000000000000017) (0.43, 0.37000000000000016) (0.44, 0.36000000000000015) (0.45, 0.35000000000000014) (0.46, 0.34000000000000014) (0.47000000000000003, 0.3300000000000001) (0.48, 0.3300000000000001) (0.49, 0.3200000000000001) (0.5, 0.3100000000000001) (0.51, 0.3000000000000001) (0.52, 0.2900000000000001) (0.53, 0.2800000000000001) (0.54, 0.2700000000000001) (0.55, 0.26000000000000006) (0.56, 0.24000000000000007) (0.5700000000000001, 0.23000000000000007) (0.58, 0.23000000000000007) (0.59, 0.22000000000000006) (0.6, 0.21000000000000005) (0.61, 0.20000000000000004) (0.62, 0.19000000000000003) (0.63, 0.18000000000000002) (0.64, 0.17) (0.65, 0.16) (0.66, 0.15) (0.67, 0.13999999999999999) (0.68, 0.12999999999999998) (0.6900000000000001, 0.11999999999999998) (0.7000000000000001, 0.10999999999999999) (0.71, 0.09999999999999999) (0.72, 0.09) (0.73, 0.08) (0.74, 0.07) (0.75, 0.060000000000000005) (0.76, 0.05) (0.77, 0.04) (0.78, 0.03) (0.79, 0.02) (0.8, 0.01)
  };
  % BFGS inexact P1
  \addplot+[color=\inexactbfgscolor] coordinates {
  (0.01, 0.05) (0.02, 0.05) (0.03, 0.060000000000000005) (0.04, 0.09999999999999999) (0.05, 0.34000000000000014) (0.06, 0.3300000000000001) (0.07, 0.3100000000000001) (0.08, 0.3000000000000001) (0.09, 0.2800000000000001) (0.1, 0.2700000000000001) (0.11, 0.25000000000000006) (0.12, 0.24000000000000007) (0.13, 0.23000000000000007) (0.14, 0.21000000000000005) (0.15, 0.20000000000000004) (0.16, 0.19000000000000003) (0.17, 0.18000000000000002) (0.18, 0.17) (0.19, 0.16) (0.2, 0.15) (0.21, 0.13999999999999999) (0.22, 0.12999999999999998) (0.23, 0.11999999999999998) (0.24, 0.10999999999999999) (0.25, 0.09999999999999999) (0.26, 0.09) (0.27, 0.08) (0.28, 0.07) (0.29, 0.07) (0.3, 0.060000000000000005) (0.31, 0.05) (0.32, 0.05) (0.33, 0.04) (0.34, 0.04) (0.35000000000000003, 0.03) (0.36, 0.04) (0.37, 0.03) (0.38, 0.02) (0.39, 0.4100000000000002) (0.4, 0.4000000000000002) (0.41000000000000003, 0.3900000000000002) (0.42, 0.38000000000000017) (0.43, 0.37000000000000016) (0.44, 0.36000000000000015) (0.45, 0.35000000000000014) (0.46, 0.34000000000000014) (0.47000000000000003, 0.3300000000000001) (0.48, 0.3300000000000001) (0.49, 0.3200000000000001) (0.5, 0.3100000000000001) (0.51, 0.3000000000000001) (0.52, 0.2900000000000001) (0.53, 0.2800000000000001) (0.54, 0.2700000000000001) (0.55, 0.26000000000000006) (0.56, 0.24000000000000007) (0.5700000000000001, 0.23000000000000007) (0.58, 0.23000000000000007) (0.59, 0.22000000000000006) (0.6, 0.21000000000000005) (0.61, 0.20000000000000004) (0.62, 0.19000000000000003) (0.63, 0.18000000000000002) (0.64, 0.17) (0.65, 0.16) (0.66, 0.15) (0.67, 0.13999999999999999) (0.68, 0.12999999999999998) (0.6900000000000001, 0.11999999999999998) (0.7000000000000001, 0.10999999999999999) (0.71, 0.09999999999999999) (0.72, 0.09) (0.73, 0.08) (0.74, 0.07) (0.75, 0.060000000000000005) (0.76, 0.05) (0.77, 0.04) (0.78, 0.03) (0.79, 0.02) (0.8, 0.01)
  };
  \legend{Newton, Inexact Newton, BFGS, Inexact BFGS}
  % \end{plot}
  \end{axis}
  \end{tikzpicture}
  \caption{\Pone}
  \end{subfigure}
  \begin{subfigure}{0.49\textwidth}
    \begin{tikzpicture}
    \begin{axis}[width=\textwidth, height=5cm, xlabel=Time (s), ylabel=, tick label style={font=\footnotesize}, legend style={font=\tiny, draw=none, fill opacity=0.5, text opacity = 1,row sep=2pt},legend columns=2, no markers]
  % \begin{plot}{Time}{Maximum admissible $\Delta t$}
    % Newton P2
    \addplot+[color=\newtoncolor] coordinates {
          (0.01, 0.03) (0.02, 0.02) (0.03, 0.04) (0.04, 0.15) (0.05, 0.34000000000000014) (0.06, 0.3200000000000001) (0.07, 0.3000000000000001) (0.08, 0.2900000000000001) (0.09, 0.2800000000000001) (0.1, 0.26000000000000006) (0.11, 0.25000000000000006) (0.12, 0.24000000000000007) (0.13, 0.22000000000000006) (0.14, 0.21000000000000005) (0.15, 0.20000000000000004) (0.16, 0.18000000000000002) (0.17, 0.17) (0.18, 0.16) (0.19, 0.15) (0.2, 0.13999999999999999) (0.21, 0.12999999999999998) (0.22, 0.11999999999999998) (0.23, 0.10999999999999999) (0.24, 0.09999999999999999) (0.25, 0.09) (0.26, 0.08) (0.27, 0.08) (0.28, 0.07) (0.29, 0.060000000000000005) (0.3, 0.060000000000000005) (0.31, 0.05) (0.32, 0.04) (0.33, 0.04) (0.34, 0.03) (0.35000000000000003, 0.03) (0.36, 0.03) (0.37, 0.02) (0.38, 0.02) (0.39, 0.02) (0.4, 0.03) (0.41000000000000003, 0.3900000000000002) (0.42, 0.38000000000000017) (0.43, 0.37000000000000016) (0.44, 0.36000000000000015) (0.45, 0.35000000000000014) (0.46, 0.34000000000000014) (0.47000000000000003, 0.3300000000000001) (0.48, 0.3300000000000001) (0.49, 0.3200000000000001) (0.5, 0.3100000000000001) (0.51, 0.3000000000000001) (0.52, 0.2900000000000001) (0.53, 0.2800000000000001) (0.54, 0.2700000000000001) (0.55, 0.26000000000000006) (0.56, 0.24000000000000007) (0.5700000000000001, 0.23000000000000007) (0.58, 0.23000000000000007) (0.59, 0.22000000000000006) (0.6, 0.21000000000000005) (0.61, 0.20000000000000004) (0.62, 0.19000000000000003) (0.63, 0.18000000000000002) (0.64, 0.17) (0.65, 0.16) (0.66, 0.15) (0.67, 0.13999999999999999) (0.68, 0.12999999999999998) (0.6900000000000001, 0.11999999999999998) (0.7000000000000001, 0.10999999999999999) (0.71, 0.09999999999999999) (0.72, 0.09) (0.73, 0.08) (0.74, 0.07) (0.75, 0.060000000000000005) (0.76, 0.05) (0.77, 0.04) (0.78, 0.03) (0.79, 0.02) (0.8, 0.01)};
  % Newton-inexact P2
  \addplot+[color=\inexactnewtoncolor] coordinates{
  (0.01, 0.03) (0.02, 0.03) (0.03, 0.09999999999999999) (0.04, 0.7600000000000005) (0.05, 0.34000000000000014) (0.06, 0.34000000000000014) (0.07, 0.3300000000000001) (0.08, 0.3200000000000001) (0.09, 0.3000000000000001) (0.1, 0.2900000000000001) (0.11, 0.2700000000000001) (0.12, 0.26000000000000006) (0.13, 0.25000000000000006) (0.14, 0.23000000000000007) (0.15, 0.22000000000000006) (0.16, 0.21000000000000005) (0.17, 0.20000000000000004) (0.18, 0.18000000000000002) (0.19, 0.17) (0.2, 0.16) (0.21, 0.15) (0.22, 0.13999999999999999) (0.23, 0.12999999999999998) (0.24, 0.11999999999999998) (0.25, 0.11999999999999998) (0.26, 0.10999999999999999) (0.27, 0.09999999999999999) (0.28, 0.09) (0.29, 0.09) (0.3, 0.08) (0.31, 0.08) (0.32, 0.07) (0.33, 0.060000000000000005) (0.34, 0.060000000000000005) (0.35000000000000003, 0.05) (0.36, 0.05) (0.37, 0.4300000000000002) (0.38, 0.03) (0.39, 0.4100000000000002) (0.4, 0.4000000000000002) (0.41000000000000003, 0.3900000000000002) (0.42, 0.38000000000000017) (0.43, 0.37000000000000016) (0.44, 0.36000000000000015) (0.45, 0.35000000000000014) (0.46, 0.34000000000000014) (0.47000000000000003, 0.3300000000000001) (0.48, 0.3300000000000001) (0.49, 0.3200000000000001) (0.5, 0.3100000000000001) (0.51, 0.3000000000000001) (0.52, 0.2900000000000001) (0.53, 0.2800000000000001) (0.54, 0.2700000000000001) (0.55, 0.26000000000000006) (0.56, 0.24000000000000007) (0.5700000000000001, 0.23000000000000007) (0.58, 0.23000000000000007) (0.59, 0.22000000000000006) (0.6, 0.21000000000000005) (0.61, 0.20000000000000004) (0.62, 0.19000000000000003) (0.63, 0.18000000000000002) (0.64, 0.17) (0.65, 0.16) (0.66, 0.15) (0.67, 0.13999999999999999) (0.68, 0.12999999999999998) (0.6900000000000001, 0.11999999999999998) (0.7000000000000001, 0.10999999999999999) (0.71, 0.09999999999999999) (0.72, 0.09) (0.73, 0.08) (0.74, 0.07) (0.75, 0.060000000000000005) (0.76, 0.05) (0.77, 0.04) (0.78, 0.03) (0.79, 0.02) (0.8, 0.01)
  };
  % BFGS P2
  \addplot+[color=\bfgscolor] coordinates {
  (0.01, 0.01) (0.02, 0.02) (0.03, 0.03) (0.04, 0.060000000000000005) (0.05, 0.09999999999999999) (0.06, 0.3300000000000001) (0.07, 0.3200000000000001) (0.08, 0.3100000000000001) (0.09, 0.3000000000000001) (0.1, 0.2900000000000001) (0.11, 0.2800000000000001) (0.12, 0.2700000000000001) (0.13, 0.25000000000000006) (0.14, 0.24000000000000007) (0.15, 0.23000000000000007) (0.16, 0.24000000000000007) (0.17, 0.22000000000000006) (0.18, 0.21000000000000005) (0.19, 0.20000000000000004) (0.2, 0.19000000000000003) (0.21, 0.18000000000000002) (0.22, 0.17) (0.23, 0.16) (0.24, 0.15) (0.25, 0.15) (0.26, 0.12999999999999998) (0.27, 0.11999999999999998) (0.28, 0.10999999999999999) (0.29, 0.09999999999999999) (0.3, 0.09) (0.31, 0.08) (0.32, 0.07) (0.33, 0.060000000000000005) (0.34, 0.05) (0.35000000000000003, 0.04) (0.36, 0.03) (0.37, 0.03) (0.38, 0.02) (0.39, 0.01) (0.4, 0.4000000000000002) (0.41000000000000003, 0.3900000000000002) (0.42, 0.38000000000000017) (0.43, 0.37000000000000016) (0.44, 0.36000000000000015) (0.45, 0.35000000000000014) (0.46, 0.34000000000000014) (0.47000000000000003, 0.3300000000000001) (0.48, 0.3300000000000001) (0.49, 0.3200000000000001) (0.5, 0.3100000000000001) (0.51, 0.3000000000000001) (0.52, 0.2900000000000001) (0.53, 0.2800000000000001) (0.54, 0.2700000000000001) (0.55, 0.26000000000000006) (0.56, 0.24000000000000007) (0.5700000000000001, 0.23000000000000007) (0.58, 0.23000000000000007) (0.59, 0.22000000000000006) (0.6, 0.21000000000000005) (0.61, 0.20000000000000004) (0.62, 0.19000000000000003) (0.63, 0.18000000000000002) (0.64, 0.17) (0.65, 0.16) (0.66, 0.15) (0.67, 0.13999999999999999) (0.68, 0.12999999999999998) (0.6900000000000001, 0.11999999999999998) (0.7000000000000001, 0.10999999999999999) (0.71, 0.09999999999999999) (0.72, 0.09) (0.73, 0.08) (0.74, 0.07) (0.75, 0.060000000000000005) (0.76, 0.05) (0.77, 0.04) (0.78, 0.03) (0.79, 0.02) (0.8, 0.01)
  };
  % BFGS inexact P2
  \addplot+[color=\inexactbfgscolor] coordinates {
  (0.01, 0.01) (0.02, 0.01) (0.03, 0.03) (0.04, 0.04) (0.05, 0.060000000000000005) (0.06, 0.08) (0.07, 0.08) (0.08, 0.2900000000000001) (0.09, 0.2800000000000001) (0.1, 0.26000000000000006) (0.11, 0.25000000000000006) (0.12, 0.24000000000000007) (0.13, 0.22000000000000006) (0.14, 0.21000000000000005) (0.15, 0.19000000000000003) (0.16, 0.18000000000000002) (0.17, 0.17) (0.18, 0.16) (0.19, 0.15) (0.2, 0.13999999999999999) (0.21, 0.12999999999999998) (0.22, 0.11999999999999998) (0.23, 0.10999999999999999) (0.24, 0.09999999999999999) (0.25, 0.09) (0.26, 0.08) (0.27, 0.08) (0.28, 0.07) (0.29, 0.060000000000000005) (0.3, 0.060000000000000005) (0.31, 0.05) (0.32, 0.04) (0.33, 0.04) (0.34, 0.03) (0.35000000000000003, 0.03) (0.36, 0.03) (0.37, 0.02) (0.38, 0.02) (0.39, 0.01) (0.4, 0.4000000000000002) (0.41000000000000003, 0.3900000000000002) (0.42, 0.38000000000000017) (0.43, 0.37000000000000016) (0.44, 0.36000000000000015) (0.45, 0.35000000000000014) (0.46, 0.34000000000000014) (0.47000000000000003, 0.3300000000000001) (0.48, 0.3300000000000001) (0.49, 0.3200000000000001) (0.5, 0.3100000000000001) (0.51, 0.3000000000000001) (0.52, 0.2900000000000001) (0.53, 0.2800000000000001) (0.54, 0.2700000000000001) (0.55, 0.26000000000000006) (0.56, 0.24000000000000007) (0.5700000000000001, 0.23000000000000007) (0.58, 0.23000000000000007) (0.59, 0.22000000000000006) (0.6, 0.21000000000000005) (0.61, 0.20000000000000004) (0.62, 0.19000000000000003) (0.63, 0.18000000000000002) (0.64, 0.17) (0.65, 0.16) (0.66, 0.15) (0.67, 0.13999999999999999) (0.68, 0.12999999999999998) (0.6900000000000001, 0.11999999999999998) (0.7000000000000001, 0.10999999999999999) (0.71, 0.09999999999999999) (0.72, 0.09) (0.73, 0.08) (0.74, 0.07) (0.75, 0.060000000000000005) (0.76, 0.05) (0.77, 0.04) (0.78, 0.03) (0.79, 0.02) (0.8, 0.01)
  };
  \legend{Newton, Inexact Newton, BFGS, Inexact BFGS}
    \end{axis}
    \end{tikzpicture}
  % \end{plot}
  \caption{\Ptwo}
  \end{subfigure}
  \caption{Heartbeat test. At each time step, the maximum $\Delta t$ that allows for convergence of the nonlinear solver is computed.}
  \label{fig:heart robust}
\end{figure}


==> plots/heart-scalab-nl-p1.tex <==
\begin{figure}
    \begin{subfigure}[b]{0.245\textwidth}
        \begin{semilogxplot}{Time (s)}{Nonlinear iterations}
        \addplot+[fill opacity=0.1, mark=none, color=\newtoncolor!40!white] table [x=t, y=nl-its, col sep=comma] {data/HEART_SCALABILITY_P1_NEWTON_1.csv};
        \addplot+[fill opacity=0.1, mark=none, color=\newtoncolor] table [x=t, y=nl-its, col sep=comma] {data/HEART_SCALABILITY_P1_NEWTON_8.csv};
        \addplot+[fill opacity=0.1, mark=none, color=\newtoncolor!40!black] table [x=t, y=nl-its, col sep=comma] {data/HEART_SCALABILITY_P1_NEWTON_32.csv};
        \legend {1 core, 8 cores, 32 cores}
      \end{semilogxplot}
      \caption{Newton}
    \end{subfigure}
    \begin{subfigure}[b]{0.245\textwidth}
        \begin{semilogxplot}{Time (s)}{}
          \addplot+[fill opacity=0.1, mark=none, color=\inexactnewtoncolor!40!white] table [x=t, y=nl-its, col sep=comma] {data/HEART_SCALABILITY_P1_NEWTON-inexact_1.csv};
          \addplot+[fill opacity=0.1, mark=none, color=\inexactnewtoncolor] table [x=t, y=nl-its, col sep=comma] {data/HEART_SCALABILITY_P1_NEWTON-inexact_8.csv};
          \addplot+[fill opacity=0.1, mark=none, color=\inexactnewtoncolor!40!black] table [x=t, y=nl-its, col sep=comma] {data/HEART_SCALABILITY_P1_NEWTON-inexact_32.csv};
          \legend {1 core, 8 cores, 32 cores}
      \end{semilogxplot}
      \caption{Inexact Newton}
    \end{subfigure}
    \begin{subfigure}[b]{0.245\textwidth}
        \begin{semilogxplot}{Time (s)}{}
          \addplot+[fill opacity=0.1, mark=none, color=\bfgscolor!40!white] table [x=t, y=nl-its, col sep=comma] {data/HEART_SCALABILITY_P1_BFGS_1.csv};
          \addplot+[fill opacity=0.1, mark=none, color=\bfgscolor] table [x=t, y=nl-its, col sep=comma] {data/HEART_SCALABILITY_P1_BFGS_8.csv};
          \addplot+[fill opacity=0.1, mark=none, color=\bfgscolor!40!black] table [x=t, y=nl-its, col sep=comma] {data/HEART_SCALABILITY_P1_BFGS_32.csv};
          \legend {1 core, 8 cores, 32 cores}
      \end{semilogxplot}
      \caption{BFGS}
    \end{subfigure}
    \begin{subfigure}[b]{0.245\textwidth}
      \begin{semilogxplot}{Time (s)}{}
        \addplot+[fill opacity=0.1, mark=none, color=\inexactbfgscolor!40!white] table [x=t, y=nl-its, col sep=comma] {data/HEART_SCALABILITY_P1_BFGS-inexact_1.csv};
        \addplot+[fill opacity=0.1, mark=none, color=\inexactbfgscolor] table [x=t, y=nl-its, col sep=comma] {data/HEART_SCALABILITY_P1_BFGS-inexact_8.csv};
        \addplot+[fill opacity=0.1, mark=none, color=\inexactbfgscolor!40!black] table [x=t, y=nl-its, col sep=comma] {data/HEART_SCALABILITY_P1_BFGS-inexact_32.csv};
        \legend {1 core, 8 cores, 32 cores}
      \end{semilogxplot}
      \caption{Inexact BFGS}
    \end{subfigure}

  \caption{Heartbeat test. Nonlinear iterations for all mettods, \Pone. }
  \label{fig:heart scalab nl p1}
\end{figure}


==> plots/heart-scalab-nl-p2.tex <==
\begin{figure}
    \begin{subfigure}[b]{0.245\textwidth}
        \begin{semilogxplot}{Time (s)}{Nonlinear iterations}
        \addplot+[fill opacity=0.1, mark=none, color=\newtoncolor!40!white] table [x=t, y=nl-its, col sep=comma] {data/HEART_SCALABILITY_P2_NEWTON_1.csv};
        \addplot+[fill opacity=0.1, mark=none, color=\newtoncolor] table [x=t, y=nl-its, col sep=comma] {data/HEART_SCALABILITY_P2_NEWTON_8.csv};
        \addplot+[fill opacity=0.1, mark=none, color=\newtoncolor!40!black] table [x=t, y=nl-its, col sep=comma] {data/HEART_SCALABILITY_P2_NEWTON_32.csv};
        \legend {1 core, 8 cores, 32 cores}
      \end{semilogxplot}
      \caption{Newton}
    \end{subfigure}
    \begin{subfigure}[b]{0.245\textwidth}
        \begin{semilogxplot}{Time (s)}{}
          \addplot+[fill opacity=0.1, mark=none, color=\inexactnewtoncolor!40!white] table [x=t, y=nl-its, col sep=comma] {data/HEART_SCALABILITY_P2_NEWTON-inexact_1.csv};
          \addplot+[fill opacity=0.1, mark=none, color=\inexactnewtoncolor] table [x=t, y=nl-its, col sep=comma] {data/HEART_SCALABILITY_P2_NEWTON-inexact_8.csv};
          \addplot+[fill opacity=0.1, mark=none, color=\inexactnewtoncolor!40!black] table [x=t, y=nl-its, col sep=comma] {data/HEART_SCALABILITY_P2_NEWTON-inexact_32.csv};
          \legend {1 core, 8 cores, 32 cores}
      \end{semilogxplot}
      \caption{Inexact Newton}
    \end{subfigure}
    \begin{subfigure}[b]{0.245\textwidth}
        \begin{semilogxplot}{Time (s)}{}
          \addplot+[fill opacity=0.1, mark=none, color=\bfgscolor!40!white] table [x=t, y=nl-its, col sep=comma] {data/HEART_SCALABILITY_P2_BFGS_1.csv};
          \addplot+[fill opacity=0.1, mark=none, color=\bfgscolor] table [x=t, y=nl-its, col sep=comma] {data/HEART_SCALABILITY_P2_BFGS_8.csv};
          \addplot+[fill opacity=0.1, mark=none, color=\bfgscolor!40!black] table [x=t, y=nl-its, col sep=comma] {data/HEART_SCALABILITY_P2_BFGS_32.csv};
          \legend {1 core, 8 cores, 32 cores}
      \end{semilogxplot}
      \caption{BFGS}
    \end{subfigure}
    \begin{subfigure}[b]{0.245\textwidth}
      \begin{semilogxplot}{Time (s)}{}
        \addplot+[fill opacity=0.1, mark=none, color=\inexactbfgscolor!40!white] table [x=t, y=nl-its, col sep=comma] {data/HEART_SCALABILITY_P2_BFGS-inexact_1.csv};
        \addplot+[fill opacity=0.1, mark=none, color=\inexactbfgscolor] table [x=t, y=nl-its, col sep=comma] {data/HEART_SCALABILITY_P2_BFGS-inexact_8.csv};
        \addplot+[fill opacity=0.1, mark=none, color=\inexactbfgscolor!40!black] table [x=t, y=nl-its, col sep=comma] {data/HEART_SCALABILITY_P2_BFGS-inexact_32.csv};
        \legend {1 core, 8 cores, 32 cores}
      \end{semilogxplot}
      \caption{Inexact BFGS}
    \end{subfigure}

  \caption{Heartbeat test. Nonlinear iterations for all mettods, \Ptwo. }
  \label{fig:heart scalab nl p2}
\end{figure}


==> plots/twist-perf-all.tex <==
\begin{figure}
  \begin{subfigure}[b]{0.245\textwidth}
      \begin{plot}{Dofs}{Nonlinear iterations}
      \addplot+[fill opacity=0.1, color=\newtoncolor] table [x=dofs, y=nl-its, col sep=comma] {data/result-perf-twist-Newton.csv};
      \addplot+[fill opacity=0.1, color=\inexactnewtoncolor] table [x=dofs, y=nl-its, col sep=comma] {data/result-perf-twist-Newton-inexact.csv};
      \legend {\newton, \inexactnewton}
    \end{plot}
  \end{subfigure}
  \begin{subfigure}[b]{0.245\textwidth}
      \begin{loglogplot}{Dofs}{CPU time}
      \addplot+[fill opacity=0.1, color=\newtoncolor] table [x=dofs, y=time, col sep=comma] {data/result-perf-twist-Newton.csv};
      \addplot+[fill opacity=0.1, color=\inexactnewtoncolor] table [x=dofs, y=time, col sep=comma] {data/result-perf-twist-Newton-inexact.csv};
      \legend {\newton, \inexactnewton}
    \end{loglogplot}
  \end{subfigure}
  \begin{subfigure}[b]{0.245\textwidth}
      \begin{plot}{Dofs}{Total linear its}
      \addplot+[fill opacity=0.1, color=\newtoncolor] table [x=dofs, y=tot-krylov, col sep=comma] {data/result-perf-twist-Newton.csv};
      \addplot+[fill opacity=0.1, color=\inexactnewtoncolor] table [x=dofs, y=tot-krylov, col sep=comma] {data/result-perf-twist-Newton-inexact.csv};
      \legend {\newton, \inexactnewton}
    \end{plot}
  \end{subfigure}
  \begin{subfigure}[b]{0.245\textwidth}
    \begin{plot}{Dofs}{Average linear its}
      \addplot+[fill opacity=0.1, color=\newtoncolor] table [x=dofs, y=avg-krylov, col sep=comma] {data/result-perf-twist-Newton.csv};
      \addplot+[fill opacity=0.1, color=\inexactnewtoncolor] table [x=dofs, y=avg-krylov, col sep=comma] {data/result-perf-twist-Newton-inexact.csv};
      \legend {\newton, \inexactnewton}
    \end{plot}
  \end{subfigure}
  \caption{Twist test. nonlinear iterations (top left), CPU time (top right), total (bottom left) and avergae (bottom right) linear iterations.}
  \label{fig:twist perf}
\end{figure}


==> plots/twist-scalab-all.tex <==
\begin{figure}
  \begin{subfigure}[b]{0.245\textwidth}
      \begin{semilogxplot}{Cores}{Nonlinear iterations}
      \addplot+[fill opacity=0.1, color=\newtoncolor] table [x=cores, y=nl-its, col sep=comma] {data/result-scalab-twist-Newton-P2.csv};
      \addplot+[fill opacity=0.1, color=\inexactnewtoncolor] table [x=cores, y=nl-its, col sep=comma] {data/result-scalab-twist-Newton-inexact-P2.csv};
      \legend {\newton, \inexactnewton}
    \end{semilogxplot}
  \end{subfigure}
  \begin{subfigure}[b]{0.245\textwidth}
      \begin{loglogplot}{Cores}{CPU time}
      \addplot+[fill opacity=0.1, color=\newtoncolor] table [x=cores, y=time, col sep=comma] {data/result-scalab-twist-Newton-P2.csv};
      \addplot+[fill opacity=0.1, color=\inexactnewtoncolor] table [x=cores, y=time, col sep=comma] {data/result-scalab-twist-Newton-inexact-P2.csv};
      \legend {\newton, \inexactnewton}
    \end{loglogplot}
  \end{subfigure}
  \begin{subfigure}[b]{0.245\textwidth}
      \begin{semilogxplot}{Cores}{Total linear its}
      \addplot+[fill opacity=0.1, color=\newtoncolor] table [x=cores, y=tot-krylov, col sep=comma] {data/result-scalab-twist-Newton-P2.csv};
      \addplot+[fill opacity=0.1, color=\inexactnewtoncolor] table [x=cores, y=tot-krylov, col sep=comma] {data/result-scalab-twist-Newton-inexact-P2.csv};
      \legend {\newton, \inexactnewton}
    \end{semilogxplot}
  \end{subfigure}
  \begin{subfigure}[b]{0.245\textwidth}
      \begin{semilogxplot}{Cores}{Average linear its}
      \addplot+[fill opacity=0.1, color=\newtoncolor] table [x=cores, y=avg-krylov, col sep=comma] {data/result-scalab-twist-Newton-P2.csv};
      \addplot+[fill opacity=0.1, color=\inexactnewtoncolor] table [x=cores, y=avg-krylov, col sep=comma] {data/result-scalab-twist-Newton-inexact-P2.csv};
      \legend {\newton, \inexactnewton}
    \end{semilogxplot}
  \end{subfigure}
  \caption{Twist test. Nonlinear iterations, solution time, total and average krylov iterations with respect to the number of cores.}
  \label{fig:twist scalab}
\end{figure}

